Decidable Models of Recursive Asynchronous Concurrency

Asynchronously communicating pushdown systems (ACPS) that satisfy the empty-stack constraint (a pushdown process may receive only when its stack is empty) are a popular decidable model for recursive programs with asynchronous atomic procedure calls. We study a relaxation of the empty-stack constraint for ACPS that permits concurrency and communication actions at any stack height, called the shaped stack constraint, thus enabling a larger class of concurrent programs to be modelled. We establish a close connection between ACPS with shaped stacks and a novel extension of Petri nets: Nets with Nested Coloured Tokens (NNCTs). Tokens in NNCTs are of two types: simple and complex. Complex tokens carry an arbitrary number of coloured tokens. The rules of NNCT can synchronise complex and simple tokens, inject coloured tokens into a complex token, and eject all tokens of a specified set of colours to predefined places. We show that the coverability problem for NNCTs is Tower-complete. To our knowledge, NNCT is the first extension of Petri nets, in the class of nets with an infinite set of token types, that has primitive recursive coverability. This result implies Tower-completeness of coverability for ACPS with shaped stacks.

==> figures/pdsmutex.tex <==
%!TEX root = ../main.tex
\begin{multicols}{2}
\begin{erlang}[emph={c1,c2,toResource,toClients,toServer,init,false,true,dist,redist,local,which,globalstate,ready,result}]
%%% Server
server() -> setup_network(), 
            redistribute().

setup_network() ->
  spawn(client),
  case (*) of
    True  -> setup_network();
    False -> 
      spawn(fun() -> resource(c1,c2,init) end),
      toResource ! isReady,
      receive fromResource:
         ready -> ()
      end;
  end, toClients ! task.

redistribute() ->
  receive toServer:
    redist(Task) -> toClients ! Task;
    result(Result) -> print(Result);
  end, redistribute().

%Combinator
combinator(C) ->
  receive C:
    (Res,IRes) -> 
      R = combine_results(Res,IRes),
      toServer ! R
  end,
  combinator(C).

% Resource
resource(C,C',S) ->
  receive toResource:
    which -> toClients ! C, resource(C',C,S);
    lock_req -> toClients ! locked, resource_locked(C,C',S);
  end.

resource_locked(C,C') ->
  receive toResource:
    unlock_req -> resource(C,C',S);
    X          -> resource_locked(C,C',update(S,X))
  end.

%%% Task CLIENT
client() ->
  receive toClients:
    Task -> 
      result = do_task(Task,false),
      case result of
        dist(C) -> ok;
        _       -> to_server ! result
      end;
  end, client().

do_task(Task) ->
  case decompose(Task) of
    local(Task',Int_result) -> 
      Result = do_task(Task'),
      return (combine(Result,Int_result));
    dist(Task', Int_result) -> 
      C = which_combine_resource(),
      Result = do_task(Task'),
      C ! (Result, Int_result),
      return Dist(C);
    redist(Task',Task'') ->  
      result = do_task(Task'),
      to_server ! Redist(Task''),
      return result;
  end.

combine(res,res')    -> combine_results(res,res');
combine(Dist(C),res) -> C ! res.

which_combine_resource() -> 
  resource ! which,
    receive toClients:
      Resource(r) -> return r
    end.

decompose_task(Task) -> 
  lock(toResource),
  resource ! getGlobalstate,
  ?Critical,
  receive toClients: 
    State ->
      (Result,Update) = decompose_task(Task, State)
  end,
  resource ! update(Update),
  unlock(toResource),
  return Result

lock(C)  -> ok;
lock(C) -> 
  C ! lock_req,
  receive toClients:
    locked -> ok
  end.

unlock(C) -> C ! unlock_req.

combine_results(res,res') -> ...

decompose_task(Task,state) -> ...

%%% Program Entry points
main() -> 
  spawn(server),
  spawn(fun() -> combinator(c1) end),
  spawn(fun() -> combinator(c2) end).
  
\end{erlang}
\end{multicols}

==> figures/pdsmutex_simpler.tex <==
%!TEX root = ../main.tex
\begin{figure}[t]%
\begin{minipage}{0.49\textwidth}
\begin{erlang}[emph={c1,c2,toResource,toWorkers,toDistributor,isReady,init,false,true,dist,redist,local,which,globalstate,ready,result, unlock_req, lock_req, update, locked, getState,state}]%
main() -> setup_network(), 
          redistribute().

setup_network() ->
  spawn(worker),
  case (*) of
    true  -> setup_network();
    false -> 
      spawn(res_start(init)),
      toResource ! isReady,
      receive toDistributor:
         ready -> ()
      end;
  end, toWorkers ! task.

redistribute() ->
  receive toDistributor:
    redist(Task) -> toWorkers ! Task;
    result(Result) -> print(Result);
  end, redistribute().
\end{erlang}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{erlang}[firstnumber=21,emph={c1,c2,toResource,toWorkers,toDistributor,isReady,init,false,true,dist,redist,local,which,globalstate,ready,result, unlock_req, lock_req, update, locked, getState,state}]
% Resource
res_start(S) = 
  fun() -> toDistributor ! ready, 
           resource(S) 
  end.
resource(S) ->
  receive toResource:
    lock_req -> 
      toWorkers ! locked, 
      resource_locked(S)
  end.

resource_locked(S) ->
  receive toResource:
    unlock_req -> resource(S);
    getState   -> 
      toWorkers ! state(S), 
      resource_locked(S);
    update(X)  -> resource_locked(X)
  end.
\end{erlang}
\end{minipage}
% \linebreak
\vspace{-4mm}
\caption{A resource and a task distributor.}
\label{fig:example:resource_and_distributor}
\end{figure}
%
\begin{figure}[tbh]
\begin{minipage}{0.49\textwidth}
\begin{erlang}[emph={c1,c2,toResource,toWorkers,toDistributor,init,false,true,dist,redist,local,which,globalstate,ready,result,getState,update,locked_req,locked,unlock_req,state}]%
worker() ->
  receive toWorkers:
    Task -> 
      result = do_task(Task),
      toDistributor ! result;
  end, worker().

do_task(Task) ->
  case decompose(Task) of
    local(Task',Int_result) -> 
      Result = do_task(Task'),
      Result' = 
        combine(Result,Int_result)
      return Result';
    redist(Task',Task'') ->  
      Result = do_task(Task'),
      toDistributor ! Redist(Task''),
      return Result;
  end.

combine(res,res')    -> ...
\end{erlang}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{erlang}[firstnumber=22,emph={c1,c2,toResource,toWorkers,toDistributor,init,false,true,dist,redist,local,which,globalstate,ready,result,getState,update,locked_req,locked,unlock_req,state}]%
decompose(Task) -> 
  lock(toResource),
  toResource ! getState,
  ?label("critical"),
  receive toWorkers: 
    state(State) ->
      (Result,Update) = 
        decompose_task(Task, State)
  end,
  toResource ! update(Update),
  unlock(toResource),
  return Result.

lock(C) -> 
  C ! lock_req,
  receive toWorkers:
    locked -> ()
  end.
unlock(C) -> C ! unlock_req.

decompose_task(Task,State) -> ...
\end{erlang}
\end{minipage}
\vspace{-4mm}
\caption{A worker that recursively solves tasks and shares its workload.}
\label{fig:example:worker}
\end{figure}%

==> macros_global.tex <==
% !TEX root = main.tex
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Make math break lines over commas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathchardef\breakingcomma\mathcode`\,
{\catcode`,=\active
  \gdef,{\breakingcomma\discretionary{}{}{}}
}
\newcommand{\commabr}[1]{\mathcode`\,=\string"8000 #1}
%----------------------------------------------------------------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% discretionary linebreak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\discn}{\discretionary{}{}{}}
%----------------------------------------------------------------------------------------------------------------------


\gdef\negtinyspace{\mkern-1.625mu}

%General
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Adding label to items
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\mycite@label{}%
\let\myitem\item%
\renewcommand{\item}{%
\@ifnextchar(%
{\myciteitem}%
{\myitem}%
}%
\gdef\myciteitem(#1){%
\@ifnextchar[%
{\gdef\mycite@label{#1}%
\mycitefullitem}%
{\myitem\label{#1}}%
}%
\newcommand{\mycitefullitem}[1][]{%
\myitem[#1]\label{\mycite@label}}%
%
%----------------------------------------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Algorithm environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{myalgorithm}{%
\begingroup%
\removelatexerror%
\begin{algorithm}[H]%
  \SetAlgoNoLine\ % 
  \SetKwProg{Fn}{proc}{\string:}{}%
}{%
\end{algorithm}%
\endgroup%
}
\newlength{\myalgorithmleft}
\setlength{\myalgorithmleft}{-1em}
\newcommand{\myalgorithminline}[2][0.185\textwidth]{%
\hbox to #1{\hspace{\myalgorithmleft}\ensuremath{\text{%
\begin{myalgorithm}%
  #2
\end{myalgorithm}%
}}}}
%----------------------------------------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Caligraphic font macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\call}{\ensuremath{\ell}}
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calc}{\ensuremath{\mathpzc{c}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
%----------------------------------------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Set/Multiset operations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\oldcomplement\complement
\renewcommand{\complement}[1][]{{#1}^{\mathsf{c}}}
% \let\my@complement\complement
% \renewcommand{\complement}[1]{#1^{\my@complement}}
\newcommand{\disjointunion}[0]{\dunion}
\newcommand{\disunion}{\dunion}
\newcommand{\dunion}{+}
\newcommand{\Dunion}{\Sum}
\newcommand{\intersect}[0]{\cap}
\newcommand{\bigunion}{\Union}
\newcommand{\union}{\cup}
\newcommand{\inters}{\cap}
\newcommand{\Union}{\bigcup}
\newcommand{\Inters}{\bigcap}
\newcommand{\Intersect}{\bigcap}
\newcommand{\Intersection}{\bigcap}
\newcommand\makeset[1]{{ {\{} #1{\}} }}
\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\varset}[1]{\{ #1 \}}
\newcommand{\mset}[1]{\ensuremath{\left[#1\right]}}
\newcommand{\varmset}[1]{\ensuremath{[#1]}}
\newcommand{\range}[1]{\ensuremath{\angle{#1}}}
\newcommand{\varrange}[1]{\ensuremath{\varangle{#1}}}
\newcommand{\Oplus}{\ensuremath{\bigoplus}}
\newcommand{\bigslant}[2]{{\raisebox{.15em}{$#1$}\hspace{-1mm}\left/\raisebox{-.15em}{$#2$}\right.}}
%----------------------------------------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Set/Multiset names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Int}{\mathbb{Z}}
\renewcommand{\P}{\powerset}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\ifxetex
  \renewcommand{\M}{\mathbb{M}}
\else
  \newcommand{\M}{\mathbb{M}}
\fi
\newcommand{\exM}[0]{\ensuremath{\overline{\M}}}
\newcommand{\powerset}{\mathscr{P}}
\newcommand{\finpow}{\powerset_{\!\!f}}
%----------------------------------------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Function operations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\preupdate}[2]{\ensuremath{#1\left[#2\right]}}
\newcommand{\varpreupdate}[2]{\ensuremath{#1[#2]}}
\newcommand{\update}[4][]{\preupdate{#2}{#3 \mapsto #4 #1}}
\newcommand{\varupdate}[4][]{\varpreupdate{#2}{#3 \mapsto #4 #1}}
\newcommand{\partialto}{\ensuremath{\rightharpoonup}}
\newcommand{\compose}{\ensuremath{\circ}}
\newcommand{\norm}[2][]{\ensuremath{\left\|#2\right\|_{#1}}}
% \let\olddiameter\diameter
\newcommand{\prediameter}[2][]{\mathpzc{d}_{#1}#2}
\newcommand{\diameter}[2][]{\prediameter[#1]{\!\left(#2\right)}}
%----------------------------------------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Logic
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\implied}[0]{\Leftarrow}
\newcommand{\iif}{\Leftrightarrow}
% \providecommand{\implies}{\Rightarrow}
%----------------------------------------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Symbols & Math operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\slog}{\ensuremath{\operatorname{slog}}}
%\newcommand\tetration[2][2]{{^{#2}#1}}
%\newcommand\tetration[2][2]{{#1\,{\uparrow^2}\,{#2}}}
\newcommand\tetration[2][2]{{#1\,{\uparrow\!\uparrow}\,{#2}}}
\newcommand{\ceil}[1]{\ensuremath{\lceil #1\rceil}}
\newcommand{\argmin}{\ensuremath{\mathop{\text{argmin}}}}
\newcommand{\is}{\mathrel{\mathop:}=}
\newcommand{\iso}{\cong}
% \newcommand{\restriction}{2}{\ensuremath{#1\big|_{#2}}}
\let\geomangle\angle
\renewcommand{\angle}[1]{\ensuremath{\left\langle #1\right\rangle}}
\newcommand{\varangle}[1]{\ensuremath{\langle #1\rangle}}
\newcommand{\paren}[1]{\ensuremath{\left(#1\right)}}
\newcommand{\varparen}[1]{(#1)}
\newcommand{\gfp}[2]{\ensuremath{\mathop{\mathit{gfp}}(#1).#2}}
\newcommand{\notmodels}{\nvDash}
\newcommand*\circled[1]{\tikz[baseline=(C.base)]\node[draw,circle,inner sep=0.25pt](C) {#1};\!}
\newcommand{\oin}{\mathrel{\raisebox{1pt}{\ensuremath{\circled{$\scriptstyle\in$}}}}}
\newcommand{\bigO}[1]{\ensuremath{O(#1)}}
\let\vect\vec
%\renewcommand{\vec}[1]{\mathbf{#1}}
\renewcommand{\vec}[1]{{\boldsymbol{{#1}}}}
% \renewcommand{\vec}[1]{\overrightarrow{#1}}
\newcommand{\sem}[1]{\left\llbracket#1\right\rrbracket}
%----------------------------------------------------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Generic Math Fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{fonttable}
% \fonttable{MnSymbolA10}
% \fonttable{MnSymbolB10}
% \fonttable{MnSymbolC10}
% \fonttable{MnSymbolD10}
\DeclareMathAlphabet{\mathcalligra}{T1}{calligra}{m}{n}

\DeclareFontFamily{U} {MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
  <-6> MnSymbolC5
  <6-7> MnSymbolC6
  <7-8> MnSymbolC7
  <8-9> MnSymbolC8
  <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12-> MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
  <-6> MnSymbolC-Bold5
  <6-7> MnSymbolC-Bold6
  <7-8> MnSymbolC-Bold7
  <8-9> MnSymbolC-Bold8
  <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12-> MnSymbolC-Bold12}{}

\DeclareSymbolFont{MnSyC} {U} {MnSymbolC}{m}{n}

\DeclareFontFamily{U} {MnSymbolD}{}
\DeclareFontShape{U}{MnSymbolD}{m}{n}{
  <-6> MnSymbolD5
  <6-7> MnSymbolD6
  <7-8> MnSymbolD7
  <8-9> MnSymbolD8
  <9-10> MnSymbolD9
  <10-12> MnSymbolD10
  <12-> MnSymbolD12}{}
\DeclareFontShape{U}{MnSymbolD}{b}{n}{
  <-6> MnSymbolD-Bold5
  <6-7> MnSymbolD-Bold6
  <7-8> MnSymbolD-Bold7
  <8-9> MnSymbolD-Bold8
  <9-10> MnSymbolD-Bold9
  <10-12> MnSymbolD-Bold10
  <12-> MnSymbolD-Bold12}{}

\DeclareSymbolFont{MnSyD} {U} {MnSymbolD}{m}{n}

\DeclareMathSymbol{\threecolon}{\mathrel}{MnSyC}{006}
\DeclareMathSymbol{\lightning}{\mathrel}{MnSyC}{161}
\DeclareMathSymbol{\neqsim}{\mathrel}{MnSyD}{130}
\DeclareMathSymbol{\nsubset}{\mathrel}{MnSyD}{216}
\DeclareMathSymbol{\nsubseteq}{\mathrel}{MnSyD}{218}
\DeclareMathSymbol{\nsupset}{\mathrel}{MnSyD}{217}
\DeclareMathSymbol{\nsupseteq}{\mathrel}{MnSyD}{219}

\DeclareMathAlphabet{\mathcalligra}{T1}{calligra}{m}{n}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathAlphabet{\mathbbold}{U}{bbold}{m}{n}

\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}
%----------------------------------------------------------------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Generic Math operators and abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \newcommand{\LeftEqNo}{\let\veqno\@@leqno}

\newcommand{\tuple}[1]{\langle\commabr{#1}\rangle}
\newcommand{\lst}[3][1]{{#2_{#1}}\ldots {#2_{#3}}}    % b_a ... b_c
\newcommand{\lstc}[3][1]{\commabr{{#2_{#1}},\ldots, {#2_{#3}}}} % b_a ,..., b_c
\newcommand{\lsts}[4]{#1_#2#4\ldots#4 #1_{#3}}        % b_a d...d b_c
\newcommand{\vct}[3][]{\ensuremath{\bar #2}} % unused args are intentional so \vect can be redef to be \lst



%\newcommand\arrlab[1]{\stackrel{#1}{\longrightarrow}}
%\newcommand\arr{\rightarrow}
%\newcommand\arrstarlab[1]{\stackrel{#1}{\longrightarrow^{\ast}}}
\newcommand\sendto[2]{{#2 \mathbin{\hbox{!}} #1}}
\newcommand\receivefrom[2]{{#2 \mathbin{\hbox{?}} #1}}
%\newcommand\seq[2]{{{#1} \vdash {#2}}}
%\newcommand{\cpst}[1]{\ensuremath{\left\llbracket#1\right\rrbracket}}
%\newcommand{\cps}[1]{\ensuremath{#1_{\text{cps}}}}

%%% Parametric extendible arrow %%%

% The following is commented out because of clash with mathtools package
%\newcommand{\xRightarrow}[2]{%
%  \ext@arrow3399{\longrightarrowtfill@}{#1}{#2}}
\newcommand{\longrightarrowtfill@}{%
  \arrowfill@\Relbar\Relbar\Rightarrow}
% \newcommand\xleftrightarrow[2][]{%
%   \ext@arrow 9999{\longleftrightarrowfill@}{#1}{#2}}
\newcommand\longleftrightarrowfill@{%
  \arrowfill@\leftarrow\relbar\rightarrow}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Symbolic interface to \to
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\oldto\to
\newlength{\@internal@to@overarrow@offset}%
\renewcommand{\to}{\internal@to}
\gdef\@internal@to@reset{%
  \gdef\@internal@to@overarrow{}%
  \gdef\@internal@to@subscript{}%  
  \gdef\@internal@to@superscript{}%  
  \setlength\@internal@to@overarrow@offset{0pt}%
}
\gdef\internal@to{\@ifnextchar[\@internal@to{\@internal@to[]}}
\gdef\@internal@to[#1]{%
    \mathrel{
      \@internal@to@reset%     
      \setkeys{internalto}{#1}%
      \xrightarrow{\@internal@to@overarrow}%
      \@internal@to@superscript%
      \@internal@to@subscript%
    }%
}
\define@key{internalto}{TS}%
  {\gdef\@internal@to@subscript{_{#1}}}
  % {\gdef\@internal@to@subscript{_{\raisebox{-0.9ex}{\hspace{-0.6ex}\ensuremath{\scriptstyle #1}}}}}
\define@key{internalto}{LTS}%
  {\gdef\@internal@to@subscript{_{#1}}}
  % {\gdef\@internal@to@subscript{_{\raisebox{-0.9ex}{\hspace{-0.6ex}\ensuremath{\scriptstyle #1}}}}}
\define@key{internalto}{label}%
  {\gdef\@internal@to@overarrow{#1}}
\define@key{internalto}{rule}%
  {\gdef\@internal@to@overarrow{#1}}
\define@key{internalto}{effect}%
  {\gdef\@internal@to@overarrow{#1}}  
\define@key{internalto}{*}[true]%
  {\gdef\@internal@to@superscript{{}\!\!^{*}}}
\define@key{internalto}{offset}[0pt]%
  {\setlength\@internal@to@overarrow@offset{#1}
    \let\old@internal@to@overarrow\@internal@to@overarrow
    \gdef\@internal@to@overarrow{\protect{\raisebox{ \@internal@to@overarrow@offset }[0pt][0pt]{ \ensuremath{ \scriptstyle{ \old@internal@to@overarrow } } }} }
  }
\define@key{internalto}{inl}[-1pt]%
  {\setlength\@internal@to@overarrow@offset{#1}
    \let\old@internal@to@overarrow\@internal@to@overarrow
    \gdef\@internal@to@overarrow{\protect{\raisebox{ \@internal@to@overarrow@offset }[0pt][0pt]{ \ensuremath{ \scriptstyle{ \old@internal@to@overarrow } } }} }
  }
%----------------------------------------------------------------------------------------------------------------------


% \let\oldto\to
% \renewcommand{\to}{\internal@to}

% \gdef\@internal@to@reset{%
%   \gdef\@internal@to@overarrow{}%
%   \gdef\@internal@to@subscript{}%  
%   \gdef\@internal@to@superscript{}%  
% }

% \gdef\internal@to{\@ifnextchar[\@internal@to{\@internal@to[]}}
% \gdef\@internal@to[#1]{%
%     \mathrel{
%       \@internal@to@reset%     
%       \setkeys{internalto}{#1}%
%       \xrightarrow{\@internal@to@overarrow}%
%       \@internal@to@superscript%
%       \@internal@to@subscript%
%     }%
% }

% \define@key{internalto}{TS}%
%   {\gdef\@internal@to@subscript{_{#1}}}
%   % {\gdef\@internal@to@subscript{_{\raisebox{-0.9ex}{\hspace{-0.6ex}\ensuremath{\scriptstyle #1}}}}}
% \define@key{internalto}{LTS}%
%   {\gdef\@internal@to@subscript{_{#1}}}
%   % {\gdef\@internal@to@subscript{_{\raisebox{-0.9ex}{\hspace{-0.6ex}\ensuremath{\scriptstyle #1}}}}}
% \define@key{internalto}{label}%
%   {\gdef\@internal@to@overarrow{#1}}
% \define@key{internalto}{effect}%
%   {\gdef\@internal@to@overarrow{#1}}  
% \define@key{internalto}{steps}%
%   {{\gdef\@internal@to@superscript{{}\!\!^{#1}}}}
% \define@key{internalto}{rule}%
%   {\gdef\@internal@to@overarrow{#1}}  
% \define@key{internalto}{*}[true]%
%   {\gdef\@internal@to@superscript{{}\!\!^{*}}}
% \define@key{internalto}{length}%
%   {\gdef\@internal@to@superscript{{}\!\!^{#1}}}


\makeatother


\newcommand{\done}[2][done]{\sout{#2} \emph{(#1)}}

==> macros_project_specific_names.tex <==
%!TEX root = main.tex
\makeatletter
\newcommand{\I}{\text{\scalebox{0.85}{$\textit{col}$}}}
\newcommand{\C}{\text{\scalebox{0.85}{$\textit{C}$}}}
\renewcommand{\S}{\text{\scalebox{0.85}{$\textit{S}$}}}

% Sets
\newcommand{\Psimple}{\ensuremath{\calP^{\S}}}
\newcommand{\Pcomplex}{\ensuremath{\calP^{\C}}}
\newcommand{\Pinner}{\ensuremath{\calP^{\I}}}
\newcommand{\Pouter}{\ensuremath{\calP^{\scriptscriptstyle O}}}
\newcommand{\colmap}{\ensuremath{\zeta}}
%\newcommand{\Configuration}{\ensuremath{\mathit{Configuration}}}
\newcommand{\Configuration}{\ensuremath{\mathit{Config}}}
\newcommand{\Msimple}[0]{\ensuremath{\calM^{\text{\scalebox{0.85}{$\textit{simple}$}}}}}
\newcommand{\Minner}[0]{\ensuremath{\calM^{\text{\scalebox{0.85}{$\textit{col}$}}}}}
\newcommand{\Mcomplex}[0]{\ensuremath{\calM^{\text{\scalebox{0.85}{$\textit{complex}$}}}}}
\newcommand{\exMsimple}[0]{\ensuremath{\overline{\calM}^{\textit{simple}}}}
\newcommand{\exMcomplex}[0]{\ensuremath{\overline{\calM}^{\textit{complex}}}}
%\newcommand{\exConfiguration}{\ensuremath{\overline{\Configuration}}}
\newcommand{\exConfiguration}{\ensuremath{\overline{\Config}}}
% \newcommand{\exMinner}[0]{\ensuremath{\overline{\calM}^{\textit{inner}}}}
\newcommand{\SimpleRules}{\ensuremath{\mathit{SimpleRules}}}
	%{\ensuremath{\Pouter \to \exM[\calV\times\Minner \union \calC]}}
\newcommand{\ComplexRules}{\ensuremath{\mathit{ComplexRules}}}
\newcommand{\TransferRules}{\ensuremath{\mathit{TransferRules}}}
%{\ensuremath{\Pcomplex \times \Pcomplex \times (\Psimple \partialto \Pinner)}}
\renewcommand{\Rules}{\ensuremath{\calR}} %\NormalRules \dunion \TransferRules}
\renewcommand{\State}{\ensuremath{\mathit{State}}}

% Relations
\newcommand{\relto}[1][]{\ensuremath{\mathrel{\xrightarrow{#1}_{\mathit{ex}}}}}
\newcommand{\vasto}[1][]{\ensuremath{\mathrel{\xrightarrow{#1}_{\mathit{VAS}}}}}
\newcommand{\zvasto}[1][]{\ensuremath{\mathrel{\xrightarrow{#1}_{\Z-\mathit{VAS}}}}}
\newcommand{\gvasto}[1][]{\ensuremath{\mathrel{\xrightarrow{#1}_{g\mathit{VAS}}}}}
\newcommand{\gzvasto}[1][]{\ensuremath{\mathrel{\xrightarrow{#1}_{g\Z-\mathit{VAS}}}}}
\newcommand{\abssimeq}[1][]{\ensuremath{\mathrel{\eqsim_{#1}}}}
\newcommand{\abssimneq}[1][]{\ensuremath{\mathrel{\neqsim_{#1}}}}
\newcommand{\abssim}[1][]{\ensuremath{\mathrel{\lesssim_{#1}}}}
\newcommand{\abssimed}[1][]{\ensuremath{\mathrel{\gtrsim_{#1}}}}
% \newcommand{\higleq}[1][\calA]{\ensuremath{\leq_{\text{Hig}}}}
% \newcommand{\higgeq}[1][\calA]{\ensuremath{\geq_{\text{Hig}}}}
% \newcommand{\higeq}[1][\calA]{\ensuremath{=_{\text{Hig}}}}
\newcommand{\higleq}[1][\calA]{\ensuremath{\leq_{{#1}^*}}}
\newcommand{\higgeq}[1][\calA]{\ensuremath{\geq_{{#1}^*}}}
\newcommand{\higeq}[1][\calA]{\ensuremath{=_{{#1}^*}}}

% Functions
\newcommand{\select}[2]{\ensuremath{\mathit{select}(#1,#2)}}
\newcommand{\splitdef}[2]{\ensuremath{\mathit{splitdef}(#1,#2)}}
\newcommand{\rank}{\ensuremath{\mathop{\mathit{rank}}\nolimits}}
\newcommand{\SCC}{\ensuremath{\mathop{\mathit{SCC}}\nolimits}}
\newcommand{\Expr}{\ensuremath{\mathop{\mathit{Expr}}}}
\renewcommand{\dist}[4][]{\ensuremath{\mathit{dist}^{#1}_{#4}(#2,#3)}}
\renewcommand{\budget}{\ensuremath{\mathop{\mathit{budget}}\nolimits}}
\newcommand{\tauextend}[1]{\ensuremath{\mathop{\tau}(#1)}}
\newcommand{\nuextend}[1]{\ensuremath{\mathop{\nu}(#1)}}
\newcommand{\moveextend}[1]{\ensuremath{#1\mathop{++}}}
\newcommand{\consextend}[2]{\ensuremath{#1\mathop{:}#2}}
\newcommand{\newtrack}[2][\large]{\ensuremath{\texttt{#1[}#2\texttt{#1]}}}

% Auxillary
\newcommand{\workingname}{\emph{(WORKING NAME)}}

% Lower Bound Specific
\newcommand{\inc}[1]{\ensuremath{#1\texttt{++}}}
\newcommand{\dec}[1]{\ensuremath{#1\texttt{--}}}
\newcommand{\reset}[1]{\ensuremath{\mathit{reset}(#1)}}
\newcommand{\iszero}[1]{\ensuremath{\mathit{iszero}(#1)}}
\newcommand{\isequal}[2]{\ensuremath{\mathit{isequal}(#1,#2)}}
\newcommand{\ismax}[1]{\ensuremath{\mathit{ismax}(#1)}}
\newcommand{\deactivate}[2][]{\ensuremath{\mathit{deactivate}#1(#2)}}
\newcommand{\activate}[1]{\ensuremath{\mathit{activate}(#1)}}
\newcommand{\ismaxandreset}[1]{\ensuremath{\mathit{ismax\&reset}(#1)}}
\newcommand{\goto}[1]{\ensuremath{\mathop{\mathbf{goto}} #1}}
\newcommand{\gotoor}[2]{\ensuremath{\mathop{\mathbf{goto}} #1 \mathrel{\mathbf{or}} #2}}
\newcommand{\gosub}[1]{\ensuremath{\mathop{\mathbf{gosub}} #1}}
\newcommand{\returnto}[3]{\ensuremath{\mathop{\mathbf{return}} \mathop{\mathbf{to}} #1 \mathop{\mathbf{release}} #2; #3}}
\newcommand{\for}[3]{\ensuremath{\mathop{\mathbf{for}} #1 \mathop{\mathbf{to}} 
#2; #3}}
\newcommand{\while}[1]{\ensuremath{\mathop{\mathbf{while}} (#1) \mathop{\mathbf{do}}}}
\newcommand{\halt}[0]{\ensuremath{\mathop{\mathbf{halt}}}}
\newcommand{\test}[2][0]{\ensuremath{%
	\mathop{\mathtt{test}}\nolimits_{#1}(#2)}%
	}
\newcommand{\otest}[6][0]{\ensuremath{%
	\mathop{\overline{\mathtt{test}}}\nolimits_{#1}(#2,#3,#4,#5,#6)}%
	}
\newcommand{\otesta}[6]{\ensuremath{%
	\mathop{{}^{[]}\overline{\mathtt{test}}}\nolimits_{0}(#1,#2,#3,#4,#5,#6)}%
	}	
\newcommand{\DEC}[1][k]{\ensuremath{\mathop{\mathbf{DEC}_{#1}}}}
\newlength{\tablength}
\setlength{\tablength}{0.4cm}

\newcommand{\tab}[1][1]{\hspace{#1\tablength}}
\newcommand{\leqlex}{\ensuremath{\leq_{\text{lex}}}}
\newcommand{\lneqlex}{\ensuremath{<_{\text{lex}}}}
\newcommand{\eqlex}{\ensuremath{=_{\text{lex}}}}
\newcommand{\geqlex}{\ensuremath{\geq_{\text{lex}}}}
\newcommand{\gneqlex}{\ensuremath{>_{\text{lex}}}}

\newcommand{\eqplex}{\ensuremath{=_{\text{plex}}}}
\newcommand{\leqplex}{\ensuremath{\leq_{\text{plex}}}}
\newcommand{\lneqplex}{\ensuremath{<_{\text{plex}}}}
\newcommand{\geqplex}{\ensuremath{\geq_{\text{plex}}}}
\newcommand{\gneqplex}{\ensuremath{>_{\text{plex}}}}
\newcommand{\decstate}{\ensuremath{S}}
\newcommand{\arrayrange}[3]{\ensuremath{#1[#2\ldots #3]}}
\newcommand{\arrayupdate}[4][]{\ensuremath{#2[#3 \mapsto #4 #1]}}
\newcommand{\arrays}[2]{\ensuremath{#2_{#1}}}
\newcommand{\ainter}[1]{\ensuremath{\sem{#1}}}

\newcommand{\valupdate}[3]{\arrayupdate{#1}{#2}{#3}}
\newcommand{\heapupdate}[4]{\ensuremath{#1\left[(#2, #3) \mapsto #4\right]}}
\newcommand{\toOP}{\ensuremath{\rightarrow_{\mathit{OP}}}}
\newcommand{\progstate}{\ensuremath{\mathit{State}}}
\newcommand{\progvars}[1][]{\ensuremath{\calV_{#1}}}
\newcommand{\progarrays}{\ensuremath{\calA}}
\newcommand{\progprocs}{\ensuremath{\mathit{Procs}}}
\newcommand{\progrules}{\ensuremath{R}}
\newcommand{\progprocrules}{\ensuremath{R^p}}
\newcommand{\proginstruct}{\ensuremath{\mathit{Instr}}}
\newcommand{\progprocvars}{\ensuremath{\mathit{ProcVars}}}
\newcommand{\proglabelvars}{\ensuremath{\mathit{ProcLabels}}}
\newcommand{\proginstructions}{\ensuremath{\mathit{Instructions}}}

\newcommand{\geqprocs}{\ensuremath{\geq_{\mathit{Procs}}}}
\newcommand{\gneqprocs}{\ensuremath{>_{\mathit{Procs}}}}

\newcommand{\valuation}{\ensuremath{\mathit{Valuation}}}
\newcommand{\heap}{\ensuremath{\mathit{Heap}}}
\newcommand{\LabelSub}{\ensuremath{\mathit{LabelSub}}}
\newcommand{\labelsub}{\ensuremath{\Phi}}
\newcommand{\varsub}{\ensuremath{\sigma}}
\newcommand{\VarSub}{\ensuremath{\mathit{VarSub}}}
\newcommand{\enumindex}[1]{\ensuremath{\mathit{index}\paren{#1}}}


\newcommand{\proginter}[2][]{\ensuremath{\sem{#2}^{\mathit{Prog}}_{#1}}}
\newcommand{\proglabels}[1][]{\ensuremath{\mathit{Label}^{#1}}}


\newcommand{\encwhatever}[4][]{\ensuremath{#1#2#3\negtinyspace\left[{\scriptstyle#4}\right]}}

\newcommand{\encwidget}[4]{\ensuremath{\mathit{Widget}(#1,#2,#3,#4)}}
\newcommand{\post}[2]{\ensuremath{\mathit{post}_{#1}\paren{#2}}}
\newif\ifhoaretrip@aligned%
\hoaretrip@alignedfalse%

\newcommand{\hoaretripaligned}{\hoaretrip@alignedtrue}
\newcommand{\hoaretripnotaligned}{\hoaretrip@alignedfalse}
\newcommand{\hoaretripsetfirstspace}[1]{\renewcommand{\hoaretripfirstspace}{\hspace{#1}}}
\newcommand{\hoaretripfirstspace}{}
\newcommand{\hoaretrip}[4][]{%\ensuremath{%
\ifhoaretrip@aligned%
\begin{aligned}
\begin{aligned}%
\else%
\fi%
\left\{#2\right\}\hoaretripfirstspace %
\ifhoaretrip@aligned%
#1\\%
#1\hspace{-4eM}%
\else%
\fi%
#3%
\ifhoaretrip@aligned%
\end{aligned}%
\hspace{+4eM}#1\\%
%
\else%
\fi%
\left\{#4\right\}%
\ifhoaretrip@aligned%
#1%
\end{aligned}%
\else%
\fi
}%}
% \newcommand{\neghoaretup}[3][]{\ensuremath{\left\{#1\right\} #2 \lightning}}
\newcommand{\neghoaretup}[3][]{\ensuremath{
\ifhoaretrip@aligned%
\begin{aligned}
\begin{aligned}%
\else%
\fi%
\left\{#2\right\} %
\ifhoaretrip@aligned%
#1\\%
#1\hspace{-4eM}%
\else%
\fi%
#3%
\ifhoaretrip@aligned%
\end{aligned}%
\hspace{+4eM}#1\\%
%
\else%
\fi%
\lightning%
\ifhoaretrip@aligned%
#1%
\end{aligned}%
\else%
\fi
}}

\newcommand{\encplace}[3][]{\encwhatever[#1]{p}{#2}{#3}}
\newcommand{\encP}[2][]{\encwhatever[#1]{{\vec{p}}}{}{#2}}
\newcommand{\encp}[2][]{\encwhatever[#1]{{p}}{}{#2}}
\newcommand{\encst}[2][]{\encwhatever[#1]{{st}}{}{#2}}
% \newcommand{\encPt}[2][]{\encwhatever[#1]{\tilde{\vec{p}}}{#2}{}}
\newcommand{\encphase}[1][]{\encP[#1]{\mathit{m}}}
\newcommand{\enclabel}[1][]{\encP[#1]{\mathit{l}}}
\newcommand{\encstate}[1][]{\encP[#1]{\State}}
\newcommand{\encvar}[1]{\encP[\ddot]{\mathit{v},{#1}}}
\newcommand{\encmodevar}[1][]{\encP[#1]{\mathit{mv}}}

\newcommand{\encphases}{\ensuremath{\mathit{Phases}}}
\newcommand{\encsimulation}{\ensuremath{\mathit{sim}}}
\newcommand{\encinternal}{\ensuremath{\mathit{int}}}
\newcommand{\encmode}{\ensuremath{\mathit{mod}}}
\newcommand{\encadminvar}{\ensuremath{\mathit{av}}}


\newcommand{\encprocvar}[1]{\ensuremath{\varsub_{#1}}}
\newcommand{\encproclabelvar}[1]{\ensuremath{\labelsub_{#1}}}
% \newcommand{\encarray}{\ensuremath{\mathit{ary}_a}}
% \newcommand{\encaddr}{\ensuremath{\mathit{adr}^I}}
\newcommand{\encaddrsimpl}{\ensuremath{\mathit{adr}^S}}
\newcommand{\encheap}{\ensuremath{\mathit{heap}}}
\newcommand{\encheapmanip}{\ensuremath{\mathit{heapmanip}}}
\newcommand{\programs}{\ensuremath{\mathit{Programs}}}
\newcommand{\nestedcolourednets}{\ensuremath{\mathit{NestedColouredTokenNets}}}
\newcommand{\numbertokenmset}[2]{\ensuremath{\mathfrak{m}_{#1}\paren{#2}}}
\newcommand{\numbersmset}[1]{\numbertokenmset{}{#1}}
\newcommand{\numbercmset}[4]{\numbertokenmset{c}{#1,#2,#3,#4}}
\newcommand{\encarray}{\ensuremath{\mathit{ary}_a}}
\newcommand{\encaddr}{\ensuremath{\mathit{adr}^I}}

\newcommand{\encrule}[3][]{\encwhatever[#1]{r}{#2}{#3}}
\newcommand{\encruleswitch}[1]{\encrule{}{\mathit{switch},#1}}

\newcommand{\encop}{\mathit{op}}
\newcommand{\encinc}{\mathit{inc}}
\newcommand{\encdec}{\mathit{dec}}
\newcommand{\encasgn}{\mathit{asgn}}
\newcommand{\encgoto}{\mathit{goto}}
\newcommand{\encmove}{\mathit{move}}
\newcommand{\enceject}{\mathit{eject}}
\newcommand{\enccreate}{\mathit{create}}
\newcommand{\encraw}{\mathit{raw}}
\newcommand{\encinject}{\mathit{inject}}
\newcommand{\encruleasgn}[1]{\encrule{}{\encasgn,#1}}
\newcommand{\encruleinc}[1]{\encrule{}{\encinc,#1}}
\newcommand{\encruledec}[1]{\encrule{}{\encdec,#1}}
\newcommand{\encrulegoto}[1]{\encrule{}{\encgoto,#1}}
\newcommand{\encruleshift}[1]{\encrule{}{\encmove,#1}}
\newcommand{\encruleeject}[1]{\encrule{}{\enceject,#1}}
\newcommand{\encruleinj}[1]{\encrule{}{\encinject,#1}}
\newcommand{\encrulecr}[1]{\encrule{}{\enccreate,#1}}
\newcommand{\encruleraw}[1]{\encrule{}{\encraw,#1}}
\newcommand{\encR}[3][]{\encwhatever[#1]{R}{#2}{#3}}
\newcommand{\encRinc}[1]{\encR{}{\encinc,#1}}
\newcommand{\encRdec}[1]{\encR{}{\encdec,#1}}
\newcommand{\encRasgn}[1]{\encR{}{\encasgn,#1}}
\newcommand{\encRgoto}[1]{\encR{}{\encgoto,#1}}
\newcommand{\encRshift}[1]{\encR{}{\encmove,#1}}
\newcommand{\encReject}[1]{\encR{}{\enceject,#1}}
\newcommand{\encRcreate}[1]{\encR{}{\enccreate,#1}}
\newcommand{\encRinject}[1]{\encR{}{\encinject,#1}}
\newcommand{\encRraw}[1]{\encR{}{\encraw,#1}}
\newcommand{\encRgotoor}[3]{\encR{}{\encgoto,#1, #2\mathop{\mathbf{or}}#3}}
\newcommand{\encWgotoor}[3]{\encW{\encgoto,#1, #2\mathop{\mathbf{or}}#3}}
\newcommand{\encW}[2][]{\encwhatever[#1]{{W}}{}{#2}}
\newcommand{\encI}[2][]{\encwhatever[#1]{{I}}{}{#2}}
\newcommand{\encS}[2][]{\encwhatever[#1]{{S}}{}{#2}}
\newcommand{\encloop}[2]{\ensuremath{\mathop{\mathit{loop}\paren{*;{#1}}} #2}}
\newcommand{\encwhile}[2]{\ensuremath{\mathop{\mathit{while}\paren{{#1}}} #2}}
\newcommand{\enccall}[3]{\ensuremath{#1()\left\langle#2,#3\right\rangle }}

\newcommand{\toRt}[1][]{\ensuremath{\mathop{\xrightarrow{#1}\nolinebreak\hspace{-0.75ex}\raise 0.9ex\hbox{$\scriptstyle *$}\hspace{0.5ex}}}}
\newcommand{\toSt}[1][]{\ensuremath{\mathop{\xRightarrow{#1}\nolinebreak\hspace{-0.75ex}\raise 0.9ex\hbox{$\scriptstyle *$}\hspace{0.5ex}}}}

% \newcommand{\encinput}[1]{\ensuremath{I(#1)}}
% \newcommand{\encinputswitch}[1]{\encrule{\mathit{switch},#1}}

\newcommand{\ztest}{\mathit{zt}}
\newcommand{\eqtest}{\mathit{et}}
\renewcommand{\DEC}{\mathit{DEC}}
\newcommand{\INIT}{\mathit{INIT}}
\newcommand{\adec}[2]{\mathit{dec}(#1,#2)}
\newcommand{\ainc}[2]{\mathit{inc}(#1,#2)}
\newcommand{\adecstr}[2]{\mathit{ad},#2}
\newcommand{\aincstr}[2]{\mathit{ai},#2}
\newcommand{\afdec}[2]{\mathit{dec}(\vec{a}_i)}
\newcommand{\afinc}[2]{\mathit{inc}(\vec{a}_i)}
\newcommand{\STr}[1]{\ensuremath{\mathit{STr}^{\left[#1\right]}}}
\newcommand{\st}[3][]{#2\mathop{#1{:}}#3}
\newcommand{\pst}[3][]{#2\mathop{#1{\threecolon}}#3}
\newcommand{\rst}[4][]{#2\mathop{#1{:}}#3\mapsto#4}
\newcommand{\rpst}[4][]{#2\mathop{#1{\threecolon}}#3\mapsto#4}
\newcommand{\size}{\ensuremath{\mathop{\mathit{size}}}}
\newcommand{\minst}[1]{\mathop{\text{min}{:}}\paren{#1}}

\newcommand{\encsatisfy}[5][]{\ensuremath{#2\paren{#3} #1\models #4 \in #5}}
\newcommand{\encsatempty}[3][]{\ensuremath{#2\paren{#3} #1\models \emptyset}}
\newcommand{\encrulesatisfy}[6][]{\ensuremath{#2\paren{#3} #1\models #4 \mapsto #5 \in #6}}
\newcommand{\encruleopsatisfy}[6][]{\ensuremath{#2\paren{#3} #1\models \set{#4 \mapsto #5 \mid #4 \in #6}}}
\newcommand{\encrulemove}[5][]{\ensuremath{#2 #1\models #3 #5 #4}}
\newcommand{\encrulemoveleft}[4][]{\encrulemove[#1]{#2}{#3}{#4}{\Mapsfrom}}
\newcommand{\encrulemoveright}[4][]{\encrulemove[#1]{#2}{#3}{#4}{\Mapsto}}
\newcommand{\encrulecomplexio}[6][]{\ensuremath{#2(#3) #1\models #4 #6 #5}}
\newcommand{\encruleextract}[5][]{\encrulecomplexio[#1]{#2}{#3}{#4}{#5}{\Downarrow}}
\newcommand{\encrulecreate}[3][]{\encrulemove[#1]{#2}{\;}{#3}{\nu}}
\newcommand{\encruleinject}[5][]{\encrulecomplexio[{#1}]{#2}{#3}{#4}{#5}{\Uparrow}}
\newcommand{\encruletransform}[5][]{\ensuremath{#2 #1\models^{#3} #4 \to #5}}
\newcommand{\encruledettransform}[5][]{\ensuremath{#2 #1\models_{\text{det}}^{#3} #4 \to #5}}
\makeatother
